A Signal-Space Analysis of Spatial Self-Interference Isolation for Full-Duplex Wireless

The challenge to in-band full-duplex wireless communication is managing self-interference. Many designs have employed spatial isolation mechanisms, such as shielding or multi-antenna beamforming, to isolate the self-interference wave from the receiver. Such spatial isolation methods are effective, but by confining the transmit and receive signals to a subset of the available space, the full spatial resources of the channel be under-utilized, expending a cost that may nullify the net benefit of operating in full-duplex mode. In this paper we leverage an antenna-theory-based channel model to analyze the spatial degrees of freedom available to a full-duplex capable base station, and observe that whether or not spatial isolation out-performs time-division (i.e. half-duplex) depends heavily on the geometric distribution of scatterers. Unless the angular spread of the objects that scatter to the intended users is overlapped by the spread of objects that backscatter to the base station, then spatial isolation outperforms time division, otherwise time division may be optimal.

==> DocGraphics/FD_BS_Clusters_old.tex <==
\tikzstyle{block} = [draw,fill=KeynoteBlue!30,minimum size=2em]
\tikzstyle{bigBlock} = [draw,fill=KeynoteRed!50,minimum size=1.5em]
\tikzstyle{scatterer} = [draw,fill=gray!50,minimum size=2em]
\tikz[auto, decoration={
  markings,
  mark=at position 1.0 with {\arrow{>}}}
]{
\coordinate (T1) at (-3,0);
\coordinate (R1) at (-1,4);
\coordinate (T2) at (1,4);
\coordinate (R2) at (3,0);
%
\node [circle,draw,KeynoteBlue] (S11) at (-1.2,1.3) [minimum size=60pt] {};
\node [circle,draw,KeynoteRed] (S12) at (0.2,2.1) [minimum size=60pt] {};
\node [circle,draw,KeynoteGreen] (S22) at (1,1.2) [minimum size=60pt] {};
%
\draw[KeynoteBlue] (T1) -- (tangent cs:node=S11,point={(T1)},solution=1);
\draw[KeynoteBlue] (T1) -- (tangent cs:node=S11,point={(T1)},solution=2);
%
\draw[KeynoteBlue] (R1) -- (tangent cs:node=S11,point={(R1)},solution=1);
\draw[KeynoteBlue] (R1) -- (tangent cs:node=S11,point={(R1)},solution=2);
%
%
\draw[KeynoteRed] (T2) -- (tangent cs:node=S12,point={(T2)},solution=1);
\draw[KeynoteRed] (T2) -- (tangent cs:node=S12,point={(T2)},solution=2);
%
\draw[KeynoteRed] (R1) -- (tangent cs:node=S12,point={(R1)},solution=1);
\draw[KeynoteRed] (R1) -- (tangent cs:node=S12,point={(R1)},solution=2);
%
\draw[KeynoteGreen] (T2) -- (tangent cs:node=S22,point={(T2)},solution=1);
\draw[KeynoteGreen] (T2) -- (tangent cs:node=S22,point={(T2)},solution=2);
%
\draw[KeynoteGreen] (R2) -- (tangent cs:node=S22,point={(R2)},solution=1);
\draw[KeynoteGreen] (R2) -- (tangent cs:node=S22,point={(R2)},solution=2);
%
%
\node[KeynoteBlue] at ($(S11.center)!40pt!(T1)$) {$\ElevT{11}$};
\node[KeynoteBlue] at ($(S11.center)!38pt!(R1)$) {$\ElevR{11}$};
%
\node[KeynoteRed] at ($(S12.center)!40pt!(T2)$) {$\ElevT{12}$};
\node[KeynoteRed] at ($(S12.center)!40pt!(R1)$) {$\ElevR{12}$};
\node[KeynoteGreen] at ($(S22.center)!38pt!(T2)$) {$\ElevT{22}$};
\node[KeynoteGreen] at ($(S22.center)!40pt!(R2)$) {$\ElevR{22}$};
%
\path (T1)+(-0.25,-0.25) node {$T_1$}
(T2)+(0,+0.25) node {$T_2$}
(R1)+(0,+0.25) node {$R_1$}
(R2)+(+0.25,-0.25) node {$R_2$};
%
\node at ($(R1)!0.5!(T2)+(0,0.75)$) {\underline{FD Base Station}};
\node at ($(T1)+(0,-0.75)$) {{User 1 (Uplink)}};
\node at ($(R2)+(0,-0.75)$) {{User 2 (Downlink)}};
%
\iftoggle{ZChanModel}{}{
\node [circle,draw,KeynoteYellow] (S21) at (-0.2,1) [minimum size=50pt] {};
%
\node[KeynoteYellow] at ($(S21.center)!40pt!(T1)$) {$\ElevT{21}$};
\node[KeynoteYellow] at ($(S21.center)!40pt!(R2)$) {$\ElevR{21}$};
%
\draw[KeynoteYellow] (T1) -- (tangent cs:node=S21,point={(T1)},solution=1);
\draw[KeynoteYellow] (T1) -- (tangent cs:node=S21,point={(T1)},solution=2);
%
\draw[KeynoteYellow] (R2) -- (tangent cs:node=S21,point={(R2)},solution=1);
\draw[KeynoteYellow] (R2) -- (tangent cs:node=S21,point={(R2)},solution=2);
%
}
}
 

==> DocGraphics/FD_BS_fig.tex <==
\tikzstyle{block} = [draw,fill=KeynoteBlue!30,minimum size=2em]
\tikzstyle{bigBlock} = [draw,fill=KeynoteRed!50,minimum size=1.5em]
\tikzstyle{scatterer} = [draw,fill=gray!50,minimum size=2em]
\tikz[auto, decoration={
  markings,
  mark=at position 1.0 with {\arrow{>}}}
]{
\path (0,0)  node (ArrayOneTx)  [ellipse,draw, minimum height = 5em, minimum width = 3em, rotate=-30, fill=KeynoteBlue, nearly transparent]  {$$} 
+(0,-1.2) node {{User 1 (Uplink)}}
+(0,-.4) node {$\bullet\vect{p}_1$}
(ArrayOneTx.center)+(-1,0) node {$\ArrayOneTx$}
;
\path (4.5,4) node (ArrayTwoTx) [ellipse,draw, minimum height = 5em, minimum width = 6em, fill=KeynoteRed, nearly transparent]  {$$}
+(-1,1.3) node {\underline{FD Base Station Rx/Tx Arrays}} 
(ArrayTwoTx.east)+(.3,.2) node {$\ArrayTwoTx$}
(ArrayTwoTx.center)+(-.4,+.3) node{$\bullet\vect{p}_2$}
;
%
%
\path (2.5,4)  node (ArrayOneRx)  [ellipse,draw, minimum height = 5em, minimum width = 6em, rotate=60, fill=KeynoteBlue, nearly transparent]  {$$}
 +(-.4,+.4) node {$\bullet\vect{q}_1$}
(ArrayOneRx.center)+(-1.2,0) node {$\ArrayOneRx$}
;
\path (7,-0) node (ArrayTwoRx) [ellipse,draw, minimum height = 3em, minimum width = 5em, fill=KeynoteRed, nearly transparent]  {$$} 
+(0,-0.8) node {{User 2 (Downlink)}}
(ArrayTwoRx.east)+(.4,0) node {$\ArrayTwoRx$}
(ArrayTwoRx.center)+(-.55,0) node{$\bullet\vect{q}_2$}
;
%
%
%
\path(3.5,2.0) node(S0) [scatterer, minimum size=1.5em] {}
+(-1.35,-.7) node(S1) [scatterer, minimum size=1.5em, rotate=-30] {}
+(3,-0.5)  node(S2) [scatterer, minimum size=1.5em, rotate=20] {}
+(2.5,+0.5)  node(S3) [scatterer, minimum size=1.5em, rotate=-20] {}
+(1.5,-0.35)  node(S4) [scatterer, minimum size=1.5em, rotate=-15] {}
+(-2,0.1)  node(S5) [scatterer, minimum size=1.5em, rotate=-15] {}
+(-3.5,0) node (ScatLabel) {{Scatterers}}
;
\draw[] (ScatLabel) -- (S5);
\draw[] (ScatLabel) -- (S1);
%
\draw[->] (ArrayOneTx.center) -- (xyz cs:x=.5); 
\draw[->] (ArrayOneTx.center) -- (xyz cs:y=.5);
\draw[->] (ArrayOneTx.center) -- (xyz cs:z=.5);
\draw[->,densely dashed] (ArrayOneTx.center) to [above] node {$\vect{k}_1$} (S1);
%
\draw[->] (ArrayOneRx.center) -- +(xyz cs:x=.5); 
\draw[->] (ArrayOneRx.center) -- +(xyz cs:y=.5);
\draw[->] (ArrayOneRx.center) -- +(xyz cs:z=.5);
\draw[->,densely dashed] (ArrayOneRx.center) to [left] node  {$\vect{\kappa}_1$} (S1);
%%
\draw[->] (ArrayTwoTx.center) -- +(xyz cs:x=.5); 
\draw[->] (ArrayTwoTx.center) -- +(xyz cs:y=.5);
\draw[->] (ArrayTwoTx.center) -- +(xyz cs:z=.5);
\draw[->,densely dashed] (ArrayTwoTx.center) to [right] node {$\vect{k}_2$} (S4);
%
\draw[->] (ArrayTwoRx.center) -- +(xyz cs:x=.5); 
\draw[->] (ArrayTwoRx.center) -- +(xyz cs:y=.5);
\draw[->] (ArrayTwoRx.center) -- +(xyz cs:z=.5);
\draw[->,densely dashed] (ArrayTwoRx.center) to node [above] {$\vect{\kappa}_2$} (S4);
%
%
}
%controls (0,1) and (1,0) 

==> DocGraphics/GenieModel.tex <==
\tikzstyle{block} = [draw,fill=KeynoteBlue!30,minimum size=2em]
\tikzstyle{bigBlock} = [draw,fill=KeynoteRed!50,minimum size=1.5em]
\tikzstyle{scatterer} = [draw,fill=gray!50,minimum size=2em]
\tikz[auto, decoration={
  markings,
  mark=at position 1.0 with {\arrow{>}}}
]{
%
\path (0,1) node (T1) {$\stackrel[\infty]{}{T_1}$};
%
\path (0,-1) node (T2) {$\stackrel[\SizeTwoTxPrime]{}{T_2}$};
%
\path (6,1) node (R1) {$\stackrel[\SizeOneRxPrime]{}{R_1}$};
%
\path (6,-1) node (R2) {$\stackrel[\infty]{}{R_2}$};
%
\path 
%(3,0) node  [circle ,draw, minimum size = 4em] (S11) {}
%(2.5,0.5) node  [circle ,draw, minimum size = 2.5em] (S12) {}
(3,0) node  [circle ,draw, minimum size = 4em] (S21) {}
%(3,0) node  [circle ,draw, minimum size = 4em] (S22) {}
;  
%%
\draw (T2.east) to node {} (S21.north west) {}
(T2.east) to node {} (S21.south) {};
\path (S21.west)+(-.5,-.45) node {$\Omega_{2}^{(t)}$};
\draw (R1.west) to node {} (S21.north) {}
(R1.west) to node {} (S21.south east) {};
\path (S21.east)+(.5,.45) node {$\Omega_{1}^{(r)}$};
%
\draw (T1.east) to node {} (S21.north) {}
(T1.east) to node {} (S21.south west) {};
%\path (S21.west)+(.5,.45) node {$\Omega_{2}^{(t)}$};
\draw (R2.west) to node {} (S21.north east) {}
(R2.west) to node {} (S21.south) {};
%
%\draw (T1.east) to node {} (S12.north) {}
%(T1.east) to node {} (S12.south west) {};
%%\path (S21.west)+(.5,.45) node {$\Omega_{2}^{(t)}$};
%\draw (R2.west) to node {} (S12.north east) {}
%(R2.west) to node {} (S12.south) {};
%\path (S21.east)+(.5,.45) node {$\Omega_{1}^{(r)}$};
%%
}


==> DocGraphics/ZChanClustersColored.tex <==
\tikzstyle{block} = [draw,fill=KeynoteBlue!30,minimum size=2em]
\tikzstyle{bigBlock} = [draw,fill=KeynoteRed!50,minimum size=1.5em]
\tikzstyle{scatterer} = [draw,fill=gray!50,minimum size=2em]
\tikz[auto, decoration={
  markings,
  mark=at position 1.0 with {\arrow{>}}}
]{
\coordinate (T1) at (-3,1);
\coordinate (R1) at (3,1);
\coordinate (T2) at (-3,-1);
\coordinate (R2) at (3,-1);
%
\node [circle,draw,KeynoteBlue] (S11) at (0,1) [minimum size=50pt] {};
%\node [circle,draw,KeynoteYellow] (S21) at (-.5,.5) [minimum size=30pt] {};
\node [circle,draw,KeynoteRed] (S12) at (+.5,0) [minimum size=50pt] {};
\node [circle,draw,KeynoteGreen] (S22) at (.5,-0.8) [minimum size=50pt] {};
%
\draw[KeynoteBlue] (T1) -- (tangent cs:node=S11,point={(T1)},solution=1);
\draw[KeynoteBlue] (T1) -- (tangent cs:node=S11,point={(T1)},solution=2);
%
\draw[KeynoteBlue] (R1) -- (tangent cs:node=S11,point={(R1)},solution=1);
\draw[KeynoteBlue] (R1) -- (tangent cs:node=S11,point={(R1)},solution=2);
%%
%\draw[KeynoteYellow] (T1) -- (tangent cs:node=S21,point={(T1)},solution=1);
%\draw[KeynoteYellow] (T1) -- (tangent cs:node=S21,point={(T1)},solution=2);
%%
%\draw[KeynoteYellow] (R2) -- (tangent cs:node=S21,point={(R2)},solution=1);
%\draw[KeynoteYellow] (R2) -- (tangent cs:node=S21,point={(R2)},solution=2);
%
%
\draw[KeynoteRed] (T2) -- (tangent cs:node=S12,point={(T2)},solution=1);
\draw[KeynoteRed] (T2) -- (tangent cs:node=S12,point={(T2)},solution=2);
%
\draw[KeynoteRed] (R1) -- (tangent cs:node=S12,point={(R1)},solution=1);
\draw[KeynoteRed] (R1) -- (tangent cs:node=S12,point={(R1)},solution=2);
%
\draw[KeynoteGreen] (T2) -- (tangent cs:node=S22,point={(T2)},solution=1);
\draw[KeynoteGreen] (T2) -- (tangent cs:node=S22,point={(T2)},solution=2);
%
\draw[KeynoteGreen] (R2) -- (tangent cs:node=S22,point={(R2)},solution=1);
\draw[KeynoteGreen] (R2) -- (tangent cs:node=S22,point={(R2)},solution=2);
%
%
\node[KeynoteBlue] at ($(S11.center)!40pt!(T1)$) {$\ClusterT{11}$};
\node[KeynoteBlue] at ($(S11.center)!40pt!(R1)$) {$\ClusterR{11}$};
%\node[KeynoteYellow] at ($(S21.center)!40pt!(T1)$) {$\ClusterT{21}$};
%\node[KeynoteYellow] at ($(S21.center)!40pt!(R2)$) {$\ClusterR{21}$};
\node[KeynoteRed] at ($(S12.center)!40pt!(T2)$) {$\ClusterT{12}$};
\node[KeynoteRed] at ($(S12.center)!40pt!(R1)$) {$\ClusterR{12}$};
\node[KeynoteGreen] at ($(S22.center)!40pt!(T2)$) {$\ClusterT{22}$};
\node[KeynoteGreen] at ($(S22.center)!40pt!(R2)$) {$\ClusterR{22}$};
%
\path (T1)+(-0.25,0) node {$T_1$}
(T2)+(-0.25,0) node {$T_2$}
(R1)+(+0.25,0) node {$R_1$}
(R2)+(+0.25,0) node {$R_2$};
}
 

==> DocGraphics/ZChanUnipolAchieve.tex <==
\begin{thm}
\label{thm:ZChanOne}
For the spatial $Z$-channel with unipolarized linear arrays, the degree-of-freedom pair $(d_1',d_2')$ is achievable, where 
\begin{align}
d_1' =&\min\left\{2\LenOneTx |\IntT{11}|, 2\LenOneRx |\IntR{11}|\right\} \\
d_2' =& \min\left\{d_{T_2},2\LenTwoRx |\IntR{22}|\right\} 1(\LenOneTx |\IntT{11}| \geq \LenOneRx |\IntR{11}|) \nonumber \\ 
 &+ \min\left\{\delta_{T_2},2\LenTwoRx |\IntR{22}|\right\} 1(\LenOneTx |\IntT{11}| < \LenOneRx |\IntR{11}|),
\end{align}
where $d_{T_2}$ and $\delta_{T_2}$ are given in (\ref{eq:dT2}-\ref{eq:deltaT2}) at the top of the following page. 


\begin{figure*}[!t]
% ensure that we have normalsize text
\normalsize
% Store the current equation number.
\setcounter{MYtempeqncnt}{\value{equation}}
% Set the equation number to one less than the one
% desired for the first equation here.
% The value here will have to changed if equations
% are added or removed prior to the place these
% equations are referenced in the main text.
\setcounter{equation}{22}
\hrulefill
\begin{align}
%
d_{T_2} =& 2 \LenTwoTx |\IntT{22} \setminus \IntT{12}|
+ 2\min \left\{ \vphantom{\left(|\IntT{12}|\right)^+}  \LenTwoTx |\IntT{22} \cap \IntT{12}|,  
(\LenTwoTx |\IntT{12}| - \LenOneRx |\IntR{12}| )^+  +   \LenOneRx |\IntR{12} \setminus \IntR{11}| \right\}^+ \label{eq:dT2}\\
%
%d_{R_2} =& \LenTwoRx |\IntR{22} \setminus \IntR{12}| + \min \left\{ {\scriptstyle \vphantom{\left(|\IntT{12}|\right)^+} \LenTwoRx |\IntR{22} \cap \IntR{12}|,
%\LenTwoRx |\IntR{21}| - \left[\LenOneRx|\IntR{11}| - \left(\LenOneTx \IntT{11} \setminus \IntT{21} + (\LenOneTx |\IntT{21}| - \LenTwoRx |\IntR{21}|)^+ \right) \right]^+ } \right\} \label{eq:d2r}\\
%
\delta_{T_2} =& 2\LenTwoRx |\IntT{22} \setminus \IntT{12}| + 2\min \left\{ {\scriptstyle\vphantom{\left(|\IntR{12}|\right)^+} \LenTwoRx |\IntT{22} \cap \IntT{12}|,
\LenTwoRx |\IntT{12}| - \left[\LenOneRx|\IntT{11}| - \left(\LenOneTx \IntR{11} \setminus \IntR{12} + (\LenTwoTx |\IntR{12}| - \LenOneRx |\IntT{12}|)^+ \right) \right]^+ } \right\} \label{eq:deltaT2}
%
%\\ \delta_{R_2} =& \LenTwoRx |\IntR{22} \setminus \IntR{21}| + \min\left\{\LenTwoRx|\IntR{22} \cap \IntR{21}|,
%(\LenTwoRx|\IntR{21}| - \LenOneTx|\IntT{21}|)^+ + \LenOneTx|\IntT{21} \setminus \IntT{11}| \right\}^+\label{eq:delta2r}
\end{align}
%
%\begin{align}
%%d_{T_1} =&  \LenOneTx |\IntT{11} \setminus \IntT{21}|
%%+ \min \left\{ \vphantom{\left(|\IntT{12}|\right)^+}  \LenOneTx |\IntT{11} \cap \IntT{21}|,  
%%\max (\LenOneTx |\IntT{21}|, \LenTwoRx |\IntR{21}| ) -  \LenTwoRx |\IntR{22} \cap \IntR{21}| \right\}^+ \label{eq:d1t}\\
%%
%d_{R_1} =& 2\LenOneRx |\IntR{11} \setminus \IntR{12}| + 2\min \left\{ {\scriptstyle \vphantom{\left(|\IntT{12}|\right)^+} \LenOneRx |\IntR{11} \cap \IntR{12}|, 
%%\right. \nonumber \\  & \left. \hspace{200pt} 
%\LenOneRx |\IntR{12}| - \left[\LenTwoRx|\IntR{22}| - \left(\LenTwoTx \IntT{22} \setminus \IntT{12} + (\LenTwoTx |\IntT{12}| - \LenOneRx |\IntR{12}|)^+ \right) \right]^+} \right\}\\
%%
%%\delta_{T_1} =& \LenOneRx |\IntT{11} \setminus \IntT{21}| + \min \left\{ {\scriptstyle \vphantom{\left(|\IntR{21}|\right)^+} \LenOneRx |\IntT{11} \cap \IntT{21}|,
%%% \right. \nonumber \\  & \left. \hspace{200pt} 
%%\LenOneRx |\IntT{21}| - \left[\LenTwoRx|\IntT{22}| - \left(\LenTwoTx \IntR{22} \setminus \IntR{21} + (\LenOneTx |\IntR{21}| - \LenTwoRx |\IntT{21}|)^+ \right) \right]^+ } \right\} \\
%%
%\delta_{R_1} =& 2\LenOneRx |\IntR{11} \setminus \IntR{12}| + 2\min\left\{\LenOneRx|\IntR{11} \cap \IntR{12}|,
%\max(\LenOneRx|\IntR{12}|, \LenTwoTx|\IntT{12}|)- \LenTwoTx|\IntT{22}\cap \IntT{12}|\right\}^+\label{eq:delta1r}
%\end{align}
% Restore the current equation number.
\setcounter{equation}{\value{MYtempeqncnt}}
% IEEE uses as a separator
\hrulefill
% The spacer can be tweaked to stop underfull vboxes.
\vspace*{4pt}
\end{figure*}
%
\end{thm}
\setcounter{equation}{24}

%\begin{align}
%\label{eq:dT2DOF}
%&d_{T_2} =  2\LenTwoTx |\IntT{22} \setminus \IntT{12}| \\
%&+2\min \left\{\!\!\!\!
%\begin{tabular}{c}
%$\LenTwoTx |\IntT{22} \cap \IntT{12}|$, \tabularnewline 
%$(\LenTwoTx |\IntT{12}| - \LenOneRx |\IntR{12}| )^+  +   \LenOneRx |\IntR{12} \setminus \IntR{11}|$
%\end{tabular} 
% \!\!\!\! \right\}, \nonumber
%\end{align}

\begin{IEEEproof}
We prove case where $\LenOneTx |\IntT{11}| \geq \LenOneRx |\IntR{11}|$. In this case we must show achievability of the degree of freedom pair
\begin{align}
d_1' &=2\LenOneRx |\IntR{11}|, \label{eq:d1PrimeCase1} \\
d_2' &=\min\left\{d_{T_2},2\LenTwoRx |\IntR{22}|\right\}, \label{eq:d2PrimeCase1}
\end{align}
where
\begin{align}
&d_{T_2} =  2\LenTwoTx |\IntT{22} \setminus \IntT{12}| + \nonumber \\
& \min \left\{ \!\!\!
\begin{tabular}{c}
$2\LenTwoTx |\IntT{22} \cap \IntT{12}|$, \tabularnewline 
$2(\LenTwoTx |\IntT{12}| - \LenOneRx |\IntR{12}| )^+  +   2\LenOneRx |\IntR{12} \setminus \IntR{11}|$
\end{tabular} 
\!\!\! \right\}. \label{eq:T2DOF}
\end{align}
The proof in the $\LenOneTx |\IntT{11}| < \LenOneRx |\IntR{11}|$ is analogous. 
%
\subsubsection{Formalizing the Channel Model}
To ease the analysis, we cast the channel model of (\ref{eq:Zchan1}-\ref{eq:Zchan2}) into the notation of linear operators on Hilbert spaces. 
Let $\TxSpace{j}$ be the space of all field distributions that transmitter $T_j$'s array of length $\LenTx$ can radiate towards the available scattering clusters, $\IntT{jj}\cup\IntT{ij}$ (both signal-of-interest and interference). In the vernacular of \cite{TsePoon05DOF_EM}, $\TxSpace{j}$ is the space of field distributions array-limited to $\LenTx$ and wavevector-limited to $\IntT{jj}\cup\IntT{ij}$.
To be precise, define $\TxSpace{j}$ to be the Hilbert space of all square-integrable functions  $X_j:\IntT{jj}\cup\IntT{ij}\rightarrow \mathbb{C}$, that can be expressed as
$$
X_j(t) = \int_{-\LenTx}^{\LenTx} \responseTx(t,p) x_j(p)\, dp,\ \quad t\in \IntT{jj}\cup\IntT{ij}
$$
for some $x_j(p),\ p\in [-\LenTx,\LenTx]$. The inner product between two member functions, $U_j,V_j\in\TxSpace{j}$, is the usual inner product
$$
\langle U_j,V_j\rangle = \int_{\IntT{jj}\cup\IntT{ij}} U_j(t)V_j^*(t)\, dt.
$$
Likewise let $\RxSpace{i}$ be the space of field distributions that can be incident on receiver $R_i$ from the available scattering clusters, $\IntR{ii}\cup\IntR{ij}$, and resolved by an array of length $\LenRx$.
More precisely, $\RxSpace{i}$ is the Hilbert space of all square-integrable functions  $Y_i:\IntR{ii}\cup\IntR{ij} \rightarrow \mathbb{C}$, that can be expressed as  
$$
Y_i(\tau) = \int_{-\LenRx}^{\LenRx} \responseRx^*(q,\tau) y_i(q)\, dq,\ \quad \tau\in \IntR{ii}\cup\IntR{ij}
$$
for some $y_i(q),\ q\in [-\LenRx,\LenRx]$, with the usual inner product. 
From \cite{TsePoon05DOF_EM}, we know that the dimension of these array-limited and wavevector-limited transmit and receive spaces are, respectively, 
\begin{align}
\dim \TxSpace{j} &= 2\LenTx |\IntT{jj}\cup\IntT{ij}|\text{, and} \\
\dim \RxSpace{i} &= 2\LenRx |\IntR{ii}\cup\IntR{ij}|.
\end{align}
%
We can think of the scattering integrals in (\ref{eq:Zchan1}-\ref{eq:Zchan2}) as operators mapping from one Hilbert space to another. Define the operator $\ScatOp{ij}:\TxSpace{j}\rightarrow\RxSpace{i}$ by
%\begin{equation}
%(\ScatOp{ij}X_j)(\tau) = \int_{\IntT{ij}} \Scat{ij}(\tau,t) X_j(t)\,dt, \qquad \tau \in \IntR{ij}
%\end{equation}
%\evanNote{Probably should be $\tau \in \IntR{ij}\cup \IntR{ii}$ to be more precise, only nonzero in $\IntR{ij}$.}
\begin{equation}
(\ScatOp{ij}X_j)(\tau) = \int_{\IntT{ij} \cup \IntT{jj}} \!\!\!\!\!\!\!\!\! \Scat{ij}(\tau,t) X_j(t)\,dt,\  \tau \in \IntR{ij}\cup \IntR{ii}.
\end{equation}
%
We can now write the channel model (\ref{eq:Zchan1}-\ref{eq:Zchan2}) in operator notation as 
\begin{align}
Y_1 &= \ScatOp{11}X_1 + \ScatOp{12}X_2 + Z_2\\
Y_2 &= \ScatOp{22}X_2 + Z_2,
\end{align}
where $X_j \in \RxSpace{j}$, for $j=1,2$ and $Y_i, Z_i \in \RxSpace{i}$ for $i=1,2$.
%where $X_1 \in \TxSpace{1}$, $X_2 \in \TxSpace{2}$, $Y_1, Z_1 \in \RxSpace{1}$, and $Y_2, Z_2 \in \RxSpace{2}$.
%
We now begin the achievability steps.



\input{AchieveSteps_v2}
%\newpage
\input{AchieveSteps_v1}


\end{IEEEproof}





==> achievePointsProof_full.tex <==
\begin{IEEEproof}
We prove case where $\LenOneTx |\IntT{11}| \geq \LenOneRx |\IntR{11}|$. In this case we must show achievability of the degree of freedom pair
\begin{align}
d_1' &=2\LenOneRx |\IntR{11}|, \label{eq:d1PrimeCase1} \\
d_2' &=\min\left\{d_{T_2},2\LenTwoRx |\IntR{22}|\right\}, \label{eq:d2PrimeCase1}
\end{align}
where
\begin{align}
&d_{T_2} =  2\LenTwoTx |\IntT{22} \setminus \IntT{12}| + \nonumber \\
& \min \left\{ \!\!\!
\begin{tabular}{c}
$2\LenTwoTx |\IntT{22} \cap \IntT{12}|$, \tabularnewline 
$2(\LenTwoTx |\IntT{12}| - \LenOneRx |\IntR{12}| )^+  +   2\LenOneRx |\IntR{12} \setminus \IntR{11}|$
\end{tabular} 
\!\!\! \right\}. \label{eq:T2DOF}
\end{align}
The proof in the $\LenOneTx |\IntT{11}| < \LenOneRx |\IntR{11}|$ is analogous. 
%
\subsubsection{Formalizing the Channel Model}
To ease the analysis, we cast the channel model of (\ref{eq:Zchan1}-\ref{eq:Zchan2}) into the notation of linear operators on Hilbert spaces. 
Let $\TxSpace{j}$ be the space of all field distributions that transmitter $T_j$'s array of length $\LenTx$ can radiate towards the available scattering clusters, $\IntT{jj}\cup\IntT{ij}$ (both signal-of-interest and interference). In the vernacular of \cite{TsePoon05DOF_EM}, $\TxSpace{j}$ is the space of field distributions array-limited to $\LenTx$ and wavevector-limited to $\IntT{jj}\cup\IntT{ij}$.
To be precise, define $\TxSpace{j}$ to be the Hilbert space of all square-integrable functions  $X_j:\IntT{jj}\cup\IntT{ij}\rightarrow \mathbb{C}$, that can be expressed as
$$
X_j(t) = \int_{-\LenTx}^{\LenTx} \responseTx(t,p) x_j(p)\, dp,\ \quad t\in \IntT{jj}\cup\IntT{ij}
$$
for some $x_j(p),\ p\in [-\LenTx,\LenTx]$. The inner product between two member functions, $U_j,V_j\in\TxSpace{j}$, is the usual inner product
$$
\langle U_j,V_j\rangle = \int_{\IntT{jj}\cup\IntT{ij}} U_j(t)V_j^*(t)\, dt.
$$
Likewise let $\RxSpace{i}$ be the space of field distributions that can be incident on receiver $R_i$ from the available scattering clusters, $\IntR{ii}\cup\IntR{ij}$, and resolved by an array of length $\LenRx$.
More precisely, $\RxSpace{i}$ is the Hilbert space of all square-integrable functions  $Y_i:\IntR{ii}\cup\IntR{ij} \rightarrow \mathbb{C}$, that can be expressed as  
$$
Y_i(\tau) = \int_{-\LenRx}^{\LenRx} \responseRx^*(q,\tau) y_i(q)\, dq,\ \quad \tau\in \IntR{ii}\cup\IntR{ij}
$$
for some $y_i(q),\ q\in [-\LenRx,\LenRx]$, with the usual inner product. 
From \cite{TsePoon05DOF_EM}, we know that the dimension of these array-limited and wavevector-limited transmit and receive spaces are, respectively, 
\begin{align}
\dim \TxSpace{j} &= 2\LenTx |\IntT{jj}\cup\IntT{ij}|\text{, and} \\
\dim \RxSpace{i} &= 2\LenRx |\IntR{ii}\cup\IntR{ij}|.
\end{align}
%
We can think of the scattering integrals in (\ref{eq:Zchan1}-\ref{eq:Zchan2}) as operators mapping from one Hilbert space to another. Define the operator $\ScatOp{ij}:\TxSpace{j}\rightarrow\RxSpace{i}$ by
%\begin{equation}
%(\ScatOp{ij}X_j)(\tau) = \int_{\IntT{ij}} \Scat{ij}(\tau,t) X_j(t)\,dt, \qquad \tau \in \IntR{ij}
%\end{equation}
%\evanNote{Probably should be $\tau \in \IntR{ij}\cup \IntR{ii}$ to be more precise, only nonzero in $\IntR{ij}$.}
\begin{equation}
(\ScatOp{ij}X_j)(\tau) = \int_{\IntT{ij} \cup \IntT{jj}} \!\!\!\!\!\!\!\!\! \Scat{ij}(\tau,t) X_j(t)\,dt,\  \tau \in \IntR{ij}\cup \IntR{ii}.
\end{equation}
%
We can now write the channel model (\ref{eq:Zchan1}-\ref{eq:Zchan2}) in operator notation as 
\begin{align}
Y_1 &= \ScatOp{11}X_1 + \ScatOp{12}X_2 + Z_2\\
Y_2 &= \ScatOp{22}X_2 + Z_2,
\end{align}
where $X_j \in \RxSpace{j}$, for $j=1,2$ and $Y_i, Z_i \in \RxSpace{i}$ for $i=1,2$.
%where $X_1 \in \TxSpace{1}$, $X_2 \in \TxSpace{2}$, $Y_1, Z_1 \in \RxSpace{1}$, and $Y_2, Z_2 \in \RxSpace{2}$.
%
We now begin the achievability steps.



\input{AchieveSteps_v2}



\end{IEEEproof}

==> converseProof_full.tex <==
\begin{thm}
\label{thm:converse}
If the degree-of-freedom pair $(d_1,d_2)$ is achievable, then $(d_1,d_2) \in \D$.
\end{thm}
\begin{IEEEproof}[Proof]
%\begin{proof}[Sketch of Proof]
Assume the degree-of-freedom pair $(d_1,d_2)$ is achievable. 
It is easy to see that constraints (\ref{eq:d1Bound}) and (\ref{eq:d2Bound}) on $\D$ must be satisfied as these are point-to-point bounds. 
It remains to show that Equation (\ref{eq:dSumBound}) of Theorem~\ref{thm:mainResult} is an outer bound on the sum degrees of freedom. 
First, let a genie increase $\LenOneTx$ and $\LenTwoRx$, the aperture size of the $T_1$ and $R_2$ arrays, towards infinity, such that the sum degrees of freedom becomes limited only by the signaling dimensions available at $T_2$ and $R_1$. Clearly, this genie will only increase the sum degrees of freedom.  

Define the union of the signal scattering interval and the interference scattering interval at $T_2$ to be $\IntT{2} = \IntT{22} \cup \IntT{12}$. 
Let a genie expand the signal scattering interval at $T_2$ from $\IntT{22}$ to $\IntTPrime{22} = \IntT{2}$ and also expand the interference scattering interval at $T_2$ from $\IntT{12}$ to $\IntTPrime{12} = \IntT{2}$. Likewise expand both the scattering intervals at $R_1$ to the union of the two clusters, i.e., $\IntRPrime{11} = \IntRPrime{12} = \IntR{11} \cup \IntR{12} = \IntR{1}$. The genie also lengthens the $T_2$ array 

%\begin{figure}[htbp]
%\begin{center}
%%\resizebox{0.5\textwidth}{!}{
%	\input{GenieModel}
%%}
%\caption{Genie-aided scattering scenario.}
%\label{fig:genie}
%\end{center}
%\end{figure}


The genie's expansion of $\IntT{22}$ and $\IntR{11}$ can only enlarge the $\D$, since it increases the available dimensions for signaling to the intended receivers. However, expanding the interference scattering clusters, $\IntT{12}$ and $\IntR{12}$, can indeed decrease $\D$ due to the added overlap with $\IntT{22}$ and $\IntT{12}$.
For example, expansion of $\IntT{12}$ into $\IntT{22} \setminus \IntT{12}$ causes the loss of $\LenTwoTx|\IntT{22} \setminus \IntT{12}|$ signaling dimensions at $T_2$ that were once independent of User 1 to now be shared with User 1. 
This cost can be compensated, however, by having the genie correspondingly lengthen $\LenOneRx$ to $\LenOneRxPrime = \LenOneRx +  \LenTwoTx \frac{|\IntT{22} \setminus \IntT{12}|} {|\IntR{1}|}$. 
Likewise the can genie lengthen $\LenTwoTx$ to $\LenTwoTxPrime = \LenTwoTx +  \LenOneRx \frac{|\IntR{11} \setminus \IntR{12}|} {|\IntT{2}|}$. 
%\evanNote{The fact that such increasing of array size compensates may not be clear.}
\evanNote{Need to make an argument here that is something like we created an extra signaling dimension that creates an orthogonal space into which receiver can project the interference}

%The genie's operation has thus transformed the original scenario shown in Figure~\ref{fig:setup} to the scenario shown in depicted in Figure~\ref{fig:genie}, and has done so such that the degree-of-freedom region of the transformed channel in Figure~\ref{fig:genie} is the same or larger than the degree of freedom region of the original channel. Note that the genie-aided channel is fully coupled, all signals incident on $R1$ are also incident on $R2$. Since the aperture sizes of the $T_1$ and $R_2$ have been allowed to approach infinity, it is only the $\LenTwoTxPrime|\IntT{2}|$ dimensions available for transmission at $T_2$ and the $\LenOneRxPrime|\IntR{1}|$ dimensions available for reception at $R_1$ Note that under the definitions above,
%The genie's operation has thus transformed our original channel model to the to 
%
%and has done so such that the degree-of-freedom region of the transformed channel in Figure~\ref{fig:genie} is the same or larger than the degree of freedom region of the original channel. 

The genie-aided channel is now fully coupled, in that all wavevector signals transmitted by $T_2$ that couple to on $R_2$ will also couple to $R_1$. And, since the aperture sizes of the $T_1$ and $R_2$ have been allowed to approach infinity, it is only the $\LenTwoTxPrime|\IntT{2}|$ dimensions available for transmission at $T_2$ and the $\LenOneRxPrime|\IntR{1}|$ dimensions available for reception at $R_1$ that constraint the sum degrees of freedom.
Note that under the definitions above,
\begin{align}
&\max(\LenTwoTxPrime|\IntT{2}|, \LenOneRxPrime|\IntR{1}|) =  \max (\LenTwoTx |\IntT{12}|,  \LenOneRx |\IntR{12}|) \nonumber \\
 &\qquad  + \LenTwoTx |\IntT{22} \setminus \IntT{12}| + \LenOneRx |\IntR{11} \setminus \IntR{12}|,  \nonumber 
\end{align}
which is the sum degree-of-freedom outer bound we wish to prove. Thus it remains to show that if show that if $(d_1,d_2)$ is achievable, then
\begin{equation}
\DoF \leq \max(\LenTwoTxPrime|\IntT{2}|, \LenOneRxPrime|\IntR{1}|) \label{eq:toShow}
\end{equation}


Consider the case in which $\LenTwoTxPrime|\IntT{2}| \geq \LenOneRxPrime|\IntR{1}|$. Increase the length of the $R_1$ array to  $\LenOneRxPrime \frac{|\IntT{2}|}{|\IntR{1}|}$, so that the dimensions for reception at $R_1$ are the same as for transmission at $T_2$. Note that this increase does not alter the upper bound of Equation (\ref{eq:toShow}) we are trying to show. Now, by hypothesis $(d_1,d_2)$ is achievable, and thus $R_1$ can decode $d_1$ streams from $T_1$ and remove the message from $T_1$ from its received signal. Since the dimensions at $R_1$ are the same as at $T_2$, $R_1$ can also decode the message from $T_2$, and thus decode $d_1 + d_2$ total streams. Since the number of dimensions available for reception at $R_1$ is $\LenTwoTxPrime|\IntT{2}|$, we have that $d_1 + d_2 \leq \LenTwoTxPrime|\IntT{2}|$. 

Now consider the case in which $\LenTwoTxPrime|\IntT{2}| < \LenOneRxPrime|\IntR{1}|$. 
By hypothesis $R_1$ can decode and remove the $d_1$ streams transmitted by $T_1$. One the message from $T_1$ is removed, $R_1$ can also decode the $d_2$ streams transmitted by $T_2$, since $d_2 \leq \LenTwoTxPrime|\IntT{2}| < \LenOneRxPrime|\IntR{1}|$. Since $R_1$ decodes $d_1 + d_2$ streams and has $\LenOneRxPrime|\IntR{1}|$ dimensions for reception, we have that $d_1 + d_2 \leq \LenOneRxPrime|\IntR{1}|$. Combining the two cases yields Equation (\ref{eq:toShow}) as desired. 

\end{IEEEproof}

==> cornerPointsProof_full.tex <==
\begin{IEEEproof}
%It is sufficient to prove only Equation (\ref{eq:corner1}) as Equation (\ref{eq:corner2}) follows by symmetry. 
%
Equations (\ref{eq:corner1})~and~(\ref{eq:corner2}) can be verified by computing the left- and right-hand sides for all combinations of the conditions 
%For example, to check equation $(\ref{eq:corner1})$, there 
%There $2$ are eight cases to be checked, 
\begin{align}
\LenOneTx|\IntT{11}|  &\lesseqgtr  \LenOneRx|\IntR{11}|,\\
%\LenOneTx|\IntT{21}|  &\lesseqgtr  \LenTwoRx|\IntR{21}|\\
\LenTwoTx|\IntT{12}|  &\lesseqgtr  \LenOneRx|\IntR{12}|,\\
\LenTwoTx|\IntT{22}|  &\lesseqgtr  \LenTwoRx|\IntR{22}|
\end{align}
and observing equality in each of the $2^3 = 8$ cases. 
%
For example, in the case where
\begin{align}
\LenOneTx|\IntT{11}|  &\geq  \LenOneRx|\IntR{11}|,\\
%\LenOneTx|\IntT{21}|  &\lesseqgtr  \LenTwoRx|\IntR{21}|\\
\LenTwoTx|\IntT{12}|  &<  \LenOneRx|\IntR{12}|,\\
\LenTwoTx|\IntT{22}|  &\geq  \LenTwoRx|\IntR{22}|,
\end{align}
we can check (\ref{eq:corner1}) by computing both sides and observing that
\begin{align}
d_1' &  = 2\LenOneRx|\IntR{11}| = \dOneMax, \\
%\end{align}
%\begin{align}
d_2' & = 2 \min\{\LenTwoRx |\IntR{22}|,\nonumber \\
	 & \qquad \LenTwoTx |\IntT{22}\setminus{\IntT{12}}| + \LenOneRx |\IntR{12} \setminus \IntR{11} |\}\\
	 & = \dSum - \dOneMax.
\end{align}
The remaining seven cases for (\ref{eq:corner1}) and the eight cases for (\ref{eq:corner2}) can be checked analogously, but are omitted for brevity. 
% that the left and right hand sides agree in  of $\SizeOneTx|\Cluster{11}{t}|  \lesseqgtr  \SizeOneRx|\Cluster{11}{r}|$, $\SizeOneTx|\Cluster{12}{t}|  \lesseqgtr  \SizeTwoRx|\Cluster{12}{r}|$, and $\SizeTwoTx|\Cluster{21}{t}|  \lesseqgtr  \SizeOneRx|\Cluster{21}{r}|$. For example in the case, $\SizeOneTx|\Cluster{11}{t}|  \geq  \SizeOneRx|\Cluster{11}{4}|$, $\SizeOneTx|\Cluster{12}{t}|  \geq  \SizeTwoRx|\Cluster{12}{r}|$, and $\SizeTwoTx|\Cluster{21}{t}|  \geq  \SizeOneRx|\Cluster{21}{r}|$, one can check that
%\begin{align}
%d_1' &= \dOneMax = \LenOneRx|\Cluster{11}{r}|, \\
%%\end{align}
%%\begin{align}
%d_2' &= \dSumMax - \dOneMax  \nonumber \\
%     &= \min \left\{ \min(\LenTwoTx|\Cluster{22}{t}|,\LenTwoRx|\Cluster{22}{r}|\nonumber ), \right. \\
%     & \hspace{35pt} \LenTwoTx|\Cluster{22}{t} \setminus \Cluster{21}{t}| 
%         + \LenTwoTx|\Cluster{21}{t}| - \LenOneRx|\Cluster{11}{r} \cap \Cluster{21}{r}|, \nonumber \\
%     & \hspace{35pt} \LenOneTx|\Cluster{11}{t} \setminus \Cluster{12}{t}| 
%         + \LenOneTx|\Cluster{12}{t}| + \LenTwoRx|\Cluster{22}{r} \setminus \Cluster{12}{r}| \nonumber \\ 
%     &\left. \hspace{45pt} - \LenOneRx|\Cluster{11}{r}|
%      \right\}.
%\end{align}
%The other seven cases can be checked analogously, but are omitted for brevity. 
\end{IEEEproof}
% Eight cases, check each one, give example for one case. 
